ML-SUPERB 2.0: Benchmarking Multilingual Speech Models Across Modeling Constraints, Languages, and Datasets

ML-SUPERB evaluates self-supervised learning (SSL) models on the tasks of language identification and automatic speech recognition (ASR). This benchmark treats the models as feature extractors and uses a single shallow downstream model, which can be fine-tuned for a downstream task. However, real-world use cases may require different configurations. This paper presents ML-SUPERB~2.0, which is a new benchmark for evaluating pre-trained SSL and supervised speech models across downstream models, fine-tuning setups, and efficient model adaptation approaches. We find performance improvements over the setup of ML-SUPERB. However, performance depends on the downstream model design. Also, we find large performance differences between languages and datasets, suggesting the need for more targeted approaches to improve multilingual ASR performance.

==> tables/downstream.tex <==
\begin{table}[!t]
    \centering
    % \caption{Investigation on downstream architectures. The number of tunable parameters are in the parentheses of the ``Param" column. + indicate the use of encoder-decoder architecture. The few-shot results are in ``CER (FS)" column. }
    \caption{Results of the downstream architecture experiments, showing the downstream model, number of model parameters (tunable parameters in parentheses), LID accuracy (ACC), aggregated CERs and few-shot CERs (FS) with standard deviations, and CERs for the worst-performing language (WL). T., C., E-B. are abbreviations for Transformer, Conformer, and E-Branchformer. +~indicates the use of the CTC-ATT framework. $\dagger$ refers to the original ML-SUPERB setting~\cite{mlsuperb}.}
    \vspace{-10pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l|c|c|ccc} 
        \toprule
        \multirow{2}{*}{Models} & \multirow{2}{*}{Method} & \multirow{2}{*}{Param. (M)} & \multirow{2}{*}{ACC} & \multicolumn{3}{c}{CER}  \\
        \cmidrule{5-7}
         & & & & Normal & FS & WL \\
        \midrule
        XLS-R  & T.\textsuperscript{$\dagger$}        & 323.7 (6.3) & 90.9 & 25.5 $\pm$ 13.5 & 33.5 $\pm$ 19.5 & 93.2 \\
        MMS    & T.\textsuperscript{$\dagger$}        & 321.8 (6.3) & 90.3 & 25.4 $\pm$ 13.7 & \textbf{30.4} $\pm$ 18.0 & \textbf{92.3}  \\
        \midrule
        \multirow{6}{*}{XLS-R } & T.        & 408.5 (91.1) & 93.7 & 21.4 $\pm$ 12.6 & 32.4 $\pm$ 19.3 & 93.3 \\
                     &  C.                   & 408.9 (91.5) & 82.3 & 25.9 $\pm$ 15.5 & 32.6 $\pm$ 18.1 & 94.5\\
                     &  E-B.                     & 409.6 (92.2) & 94.1 & 18.9 $\pm$ 12.6 & 31.4 $\pm$ 19.4 & 94.1 \\
                     \cmidrule{2-7}
                     & T.\textsuperscript{+}    & 416.0 (98.6) & 93.6  & 19.8 $\pm$ 13.5 & 32.7 $\pm$ 19.4 & 93.1 \\
                     & C.\textsuperscript{+}   & 416.3 (98.9) & 83.7 & 24.4 $\pm$ 19.9 & 33.9 $\pm$ 21.2 & 102.9 \\
                     & E-B.\textsuperscript{+}   & 417.1 (99.7)  &  94.7 & 17.6 $\pm$ 12.7 & 31.5 $\pm$ 19.6 & 93.5 \\
        \midrule
        \multirow{6}{*}{MMS}  & T.        & 406.6 (91.1) & 93.6 & 21.7 $\pm$ 13.0 & 31.1 $\pm$ 18.6 & 93.7 \\
                     &  C.                  &  407.0 (91.5) & 83.6 & 26.1 $\pm$ 17.3 & 32.1 $\pm$ 17.2 & 109.6\\
                     &  E-B.             & 407.7 (92.2) & 93.0 & 21.1 $\pm$ 12.6 & 30.5 $\pm$ 18.6 & 94.3 \\
                     \cmidrule{2-7}
                     & T.\textsuperscript{+}    & 414.1 (98.6) & 94.3 & 19.6 $\pm$ 13.5 & 31.3 $\pm$ 18.3 & 92.7 \\
                     & C.\textsuperscript{+}   & 414.4 (98.9) & 84.0 & 24.5 $\pm$ 17.8 & 33.0 $\pm$ 17.8 & 106.1 \\
                     & E-B.\textsuperscript{+}   & 415.2 (99.7)  & \textbf{95.2} & \textbf{17.4} $\pm$ 13.6 & 31.9 $\pm$ 19.3 & 93.3 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-10pt}
    \label{tab:downstream}
\end{table}

==> tables/efficient-adaptation.tex <==
\begin{table}[!t]
    \centering
    % \caption{Investigation on efficient model adaptation. The number of tunable parameters are in the parentheses of the ``Param" column. + indicate the use of encoder-decoder architecture. The few-shot results are in ``CER (FS)" column.}
    \caption{Results of the efficient model adaptation experiments, showing the method, number of model parameters (tunable parameters in parentheses), LID accuracy (ACC), aggregated CERs and few-shot CERs (FS) with standard deviations, and CERs for the worst-performing language (WL). +~indicate the use of the CTC-ATT framework. $\dagger$ refers to the original ML-SUPERB setting~\cite{mlsuperb}.}
    \vspace{-10pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l|c|c|ccc} 
        \toprule
        \multirow{2}{*}{Models} & \multirow{2}{*}{Method} & \multirow{2}{*}{Param. (M)} & \multirow{2}{*}{ACC} & \multicolumn{3}{c}{CER}  \\
        \cmidrule{5-7}
         & & & & Normal & FS & WL \\
        \midrule
        XLS-R  & -\textsuperscript{$\dagger$}        & 323.7 (6.3) & 90.9 & 25.5 $\pm$ 13.5 & 33.5 $\pm$ 19.5 & 93.2  \\
        MMS    & -\textsuperscript{$\dagger$}        & 321.8 (6.3) & 90.3 & 25.4 $\pm$ 13.7 & \textbf{30.4} $\pm$ 18.0 & \textbf{92.3}  \\
        \midrule
        \multirow{4}{*}{XLS-R } &  LoRA      & 410.1 (92.7) & \textbf{94.4} & 21.0 $\pm$ 12.5 & 32.3 $\pm$ 19.5 & 93.6 \\
                     &  Adapter                    & 411.7 (94.3) & 94.2 & 21.3 $\pm$ 12.6 & 32.8 $\pm$ 19.3 & 93.3 \\
                     \cmidrule{2-7}
                     &  LoRA\textsuperscript{+}  &   415.8 (98.4)   &  93.8 & 19.8 $\pm$ 13.6 & 32.9 $\pm$ 19.3 & 92.9 \\
                     &  Adapter\textsuperscript{+}  &  417.4 (100.0) & 93.4 & 20.2 $\pm$ 13.4 & 32.5 $\pm$ 19.3 & 93.2 \\
        \midrule
        \multirow{4}{*}{MMS}  &   LoRA             & 408.2 (92.7) & 93.5 & 22.0 $\pm$ 12.7 & 30.9 $\pm$ 17.7 & 93.7 \\
                     &   Adapter          & 409.8 (94.3) & 91.7 & 25.2 $\pm$ 12.7 & 34.8 $\pm$ 17.9  & 94.2 \\
                     \cmidrule{2-7}
                     &   LoRA\textsuperscript{+}  &   413.7 (98.4)   & 94.2 & \textbf{19.4} $\pm$ 13.3 & 32.0 $\pm$ 19.2 & 92.5 \\
                     &   Adapter\textsuperscript{+}  &  415.5 (100.0) & 92.3 & 22.6 $\pm$ 13.8 & 35.0 $\pm$ 18.5 & 93.7 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-10pt}
    \label{tab:adaptation}
\end{table}

==> tables/fine-tuning.tex <==
\begin{table}[!t]
    \centering
    % \caption{Investigation on pre-trained model fine-tuning. The number of tunable parameters are in the parentheses of the ``Param" column. + indicate the use of encoder-decoder architecture. The few-shot results are in ``CER (FS)" column.}
    \caption{Results of the fine-tuning experiments, showing the method, number of model parameters (tunable parameters in parentheses), LID accuracy (ACC), aggregated CERs and few-shot CERs (FS) with standard deviations, and CERs for the worst-performing language (WL). +~indicate the use of the CTC-ATT framework. $\dagger$ refers to the original ML-SUPERB setting~\cite{mlsuperb}.}
    \vspace{-10pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l|c|c|ccc} 
        \toprule
        \multirow{2}{*}{Models} & \multirow{2}{*}{Method} & \multirow{2}{*}{Param. (M)} & \multirow{2}{*}{ACC} & \multicolumn{3}{c}{CER}  \\
        \cmidrule{5-7}
         & & & & Normal & FS & WL \\
        \midrule
        XLS-R  & -\textsuperscript{$\dagger$}        & 323.7 (6.3) & 90.9 & 25.5 $\pm$ 13.5 & 33.5 $\pm$ 19.5 & 93.2  \\
        MMS    & -\textsuperscript{$\dagger$}        & 321.8 (6.3) & 90.3 & 25.4 $\pm$ 13.7 & 30.4 $\pm$ 18.0 & \textbf{92.3}  \\
        \midrule
        \multirow{8}{*}{XLS-R } &  1-6      & 323.7 (90.3) & 91.7 & 21.2 $\pm$ 14.3 & 28.8 $\pm$ 17.1 & 93.3 \\
                     &  9-14     & 323.7 (90.3) & 93.0 & 19.2 $\pm$ 14.4 & 30.5 $\pm$ 20.0 & 94.0 \\
                     &  19-24    & 323.7 (90.3) & 91.4 & 22.6 $\pm$ 14.6 & 31.0 $\pm$ 19.6 & 94.3 \\
                     & 1-24 & 323.7 (323.7) & 94.3 & 16.5 $\pm$ 14.2 & 28.0 $\pm$ 19.6 & 93.5 \\
                     \cmidrule{2-7}
                     &  1-6\textsuperscript{+}      & 333.4 (99.9) & 84.0 & 31.1 $\pm$ 23.4 & 34.9 $\pm$ 16.9 & 119.1 \\
                     &  9-14\textsuperscript{+}      & 333.4 (99.9) & 93.2 & 23.3 $\pm$ 19.2 & 31.6 $\pm$ 17.9 & 96.0 \\
                     &  19-24\textsuperscript{+}     & 333.4 (99.9) & 89.8 & 26.2 $\pm$ 20.3 & 31.6 $\pm$ 17.5 & 101.5\\
                     & 1-24\textsuperscript{+}   & 333.4 (333.4) & 94.1 & 17.4 $\pm$  13.7 & 28.8 $\pm$ 16.3 & 93.3   \\
        \midrule
        \multirow{8}{*}{MMS}  &  1-6      & 321.8 (90.8) & 93.8 & 19.4 $\pm$ 13.7 & 30.2 $\pm$ 19.7 & 93.8  \\
                     &  9-14                   & 321.8 (90.8) &  95.6 & \textbf{16.2} $\pm$ 12.5 & \textbf{27.2} $\pm$ 16.5 & 94.3 \\
                     &  19-24                   & 321.8 (90.8) & 93.4 & 20.1 $\pm$ 16.0 & 27.9 $\pm$ 17.1 & 96.2 \\
                     & 1-24 & 321.8 (321.8)& 87.7 & 28.1 $\pm$ 14.8 & 31.1 $\pm$ 18.1 & 92.7 \\
                     \cmidrule{2-7}
                     &  1-6\textsuperscript{+}       & 331.4 (100.5) & 93.6 & 25.9 $\pm$ 17.4 & 35.3 $\pm$ 18.8 & 93.6\\
                     &  9-14\textsuperscript{+}     & 331.4 (100.5) & \textbf{95.7} &  18.2 $\pm$ 16.0 & 28.4 $\pm$ 16.3 & 93.9 \\
                     &  19-24\textsuperscript{+}    & 331.4 (100.5) & 92.1 & 23.8 $\pm$ 22.3 & 28.1 $\pm$ 17.5 & 119.7 \\
                     & 1-24\textsuperscript{+}  & 331.4 (331.4) & 95.5 & 16.5 $\pm$ 16.4 & 29.4 $\pm$ 19.4 & 93.1 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-15pt}
    \label{tab:fine-tuning}
\end{table}

==> tables/supervised.tex <==
\begin{table}[!t]
    \centering
    % \caption{Investigation on using supervised pre-trained model. The number of tunable parameters are in the parentheses of the ``Param" column. * indicate that only encoder of the supervised model is used, while the other cases use both encoder and decoder. The few-shot results are in ``CER (FS)" column.}
    \caption{Results of the supervised model experiments, showing whether fine-tuning (FT) is performed, number of model parameters (tunable parameters in parentheses), LID accuracy (ACC), aggregated CERs and few-shot CERs (FS) with standard deviations, and CERs for the worst-performing language (WL). Asterisks indicate that only the encoder is used. $\dagger$ refers to the original ML-SUPERB setting~\cite{mlsuperb}.}
    \vspace{-10pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l|c|c|ccc} 
        \toprule
        \multirow{2}{*}{Models} & \multirow{2}{*}{FT} & \multirow{2}{*}{Param. (M)} & \multirow{2}{*}{ACC} & \multicolumn{3}{c}{CER}  \\
        \cmidrule{5-7}
         & & & & Normal & FS & WL \\
        \midrule
        XLS-R  & \xmark\textsuperscript{$\dagger$}        & 323.7 (6.3) & 90.9 & 25.5 $\pm$ 13.5 & 33.5 $\pm$ 19.5 & 93.2 \\
        MMS    & \xmark\textsuperscript{$\dagger$}        & 321.8 (6.3) & 90.3 & 25.4 $\pm$ 13.7 & 30.4 $\pm$ 18.0 & \textbf{92.3}  \\
        \midrule
        \multirow{3}{*}{Whisper } &  \xmark*  & 515.8 (91.1) & \textbf{91.7} & \textbf{21.8} $\pm$ 14.1 & \textbf{27.1} $\pm$ 13.2 & 93.4 \\
                     &  \cmark*      & 431.0 (90.7) & 83.9 & 27.5 $\pm$ 16.1 & 29.3 $\pm$ 13.4 & 93.5 \\
                     % &  Lora*      &  & \\
                     % &  Housbly*                    &  &  & \\
                     \cmidrule{2-7}
                     &  \cmark  & 762.3 (84.4) & 85.5 & 26.3 $\pm$ 20.3 & 34.4 $\pm$ 17.0 & 107.2 \\
                     % &  Lora &      &  & \\
                     % &  Housbly &   &  & \\
        \midrule
        \multirow{3}{*}{OWSM}  &  \xmark*  & 671.2 (88.4) & 77.8 & 28.3 $\pm$ 23.3 & 31.2 $\pm$ 16.9 & 99.9 \\
                     &  \cmark*      & 612.1 (88.4) & 71.0 & 25.3 $\pm$ 16.2 & 30.9 $\pm$ 16.5 & 99.7 \\
                     % &  Lora*      &  & \\
                     % &  Housbly*                    &  &  & \\
                     \cmidrule{2-7}
                     &  \cmark  & 1016.9 (100.8) & 80.5 & 40.5 $\pm$ 41.7 & 39.6 $\pm$ 24.9 & 337.6 \\
                     % &  Lora &      &  & \\
                     % &  Housbly &   &  & \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-10pt}
    \label{tab:supervised}
\end{table}
